HandyPriors: Physically Consistent Perception of Hand-Object Interactions with Differentiable Priors

Various heuristic objectives for modeling hand-object interaction have been proposed in past work. However, due to the lack of a cohesive framework, these objectives often possess a narrow scope of applicability and are limited by their efficiency or accuracy. In this paper, we propose HandyPriors, a unified and general pipeline for pose estimation in human-object interaction scenes by leveraging recent advances in differentiable physics and rendering. Our approach employs rendering priors to align with input images and segmentation masks along with physics priors to mitigate penetration and relative-sliding across frames. Furthermore, we present two alternatives for hand and object pose estimation. The optimization-based pose estimation achieves higher accuracy, while the filtering-based tracking, which utilizes the differentiable priors as dynamics and observation models, executes faster. We demonstrate that HandyPriors attains comparable or superior results in the pose estimation task, and that the differentiable physics module can predict contact information for pose refinement. We also show that our approach generalizes to perception tasks, including robotic hand manipulation and human-object pose estimation in the wild.

==> shortcuts.tex <==
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{amsmath}
\usepackage{graphicx}

\makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA

\newcommand*\xoverline[2][0.75]{%
    \sbox{\myboxA}{$\m@th#2$}%
    \setbox\myboxB\null% Phantom box
    \ht\myboxB=\ht\myboxA%
    \dp\myboxB=\dp\myboxA%
    \wd\myboxB=#1\wd\myboxA% Scale phantom
    \sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
    \setlength\mylenA{\the\wd\myboxA}%   calc width diff
    \addtolength\mylenA{-\the\wd\myboxB}%
    \ifdim\wd\myboxB<\wd\myboxA%
       \rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
    \else
        \hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
    \fi}
\makeatother

\usepackage{bm,xspace}
\usepackage{comment}
\usepackage{verbatim}
\usepackage{multirow}
\usepackage{balance}
\usepackage{url}
\usepackage{booktabs}
\usepackage{etoolbox,siunitx}
\usepackage{calc}
\usepackage{pifont,hologo}
\setlength\heavyrulewidth{0.10em}
\setlength\lightrulewidth{0.05em}
\setlength\cmidrulewidth{0.03em}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
% \usepackage{algpseudocode}

\usepackage[super]{nth}
\usepackage{nicefrac}
\sisetup{detect-weight=true,detect-inline-weight=math}
\sisetup{quotient-mode = fraction}
\sisetup{fraction-function = \nicefrac}
\robustify\bfseries


\def\aa{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\cc{\mathbf{c}}
\def\dd{\mathbf{d}}
\def\ee{\mathbf{e}}
\def\ff{\mathbf{f}}
\def\gg{\mathbf{g}}
\def\hh{\mathbf{h}}
\def\ii{\mathbf{i}}
\def\jj{\mathbf{j}}
\def\kk{\mathbf{k}}
\def\ll{\mathbf{l}}
\def\mm{\mathbf{m}}
\def\nn{\mathbf{n}}
\def\oo{\mathbf{o}}
\def\pp{\mathbf{p}}
\def\qq{\mathbf{q}}
\def\rr{\mathbf{r}}
\def\sss{\mathbf{s}}
\def\tt{\mathbf{t}}
\def\uu{\mathbf{u}}
\def\vv{\mathbf{v}}
\def\ww{\mathbf{w}}
\def\xx{\mathbf{x}}
\def\yy{\mathbf{y}}
\def\zz{\mathbf{z}}

\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CC{\mathbf{C}}
\def\DD{\mathbf{D}}
\def\EE{\mathbf{E}}
\def\FF{\mathbf{F}}
\def\GG{\mathbf{G}}
\def\HH{\mathbf{H}}
\def\II{\mathbf{I}}
\def\JJ{\mathbf{J}}
\def\KK{\mathbf{K}}
\def\LL{\mathbf{L}}
\def\MM{\mathbf{M}}
\def\NN{\mathbf{N}}
\def\OO{\mathbf{O}}
\def\PP{\mathbf{P}}
\def\QQ{\mathbf{Q}}
\def\RR{\mathbf{R}}
\def\SS{\mathbf{S}}
\def\TT{\mathbf{T}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
\def\WW{\mathbf{W}}
\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\ZZ{\mathbf{Z}}

\def\aA{\mathcal{A}}
\def\bB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\dD{\mathcal{D}}
\def\eE{\mathcal{E}}
\def\fF{\mathcal{F}}
\def\gG{\mathcal{G}}
\def\hH{\mathcal{H}}
\def\iI{\mathcal{I}}
\def\jJ{\mathcal{J}}
\def\kK{\mathcal{K}}
\def\lL{\mathcal{L}}
\def\mM{\mathcal{M}}
\def\nN{\mathcal{N}}
\def\oO{\mathcal{O}}
\def\pP{\mathcal{P}}
\def\qQ{\mathcal{Q}}
\def\rR{\mathcal{R}}
\def\sS{\mathcal{S}}
\def\tT{\mathcal{T}}
\def\uU{\mathcal{U}}
\def\vV{\mathcal{V}}
\def\wW{\mathcal{W}}
\def\xX{\mathcal{X}}
\def\yY{\mathcal{Y}}
\def\zZ{\mathcal{Z}}

\def\Ae{\mathbb{A}}
\def\Be{\mathbb{B}}
\def\Ce{\mathbb{C}}
\def\Le{\mathbb{L}}
\def\Ne{\mathbb{N}}
\def\Pe{\mathbb{P}}
\def\Qe{\mathbb{Q}}
\def\Re{\mathbb{R}}
\def\Se{\mathbb{S}}
\def\Te{\mathbb{T}}
\def\Xe{\mathbb{X}}
\def\Ye{\mathbb{Y}}
\def\Ze{\mathbb{Z}}

\def\btheta{{\bm\theta}}
\def\bzeta{{\bm\zeta}}
\def\bmu{{\bm\mu}}
\def\bZero{\mathbf{0}}
\def\bOne{\mathbf{1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{minimize}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}

\def\eps{\varepsilon}
\def\vphi{\varphi}
\def\vsigma{\varsigma}

\def\trans{^{\top}}
\def\deg{^{\circ}}

\def\th{^{\textnormal{th}}}
\def\st{^{\textnormal{st}}}
\def\nd{^{\textnormal{nd}}}

\newcommand\ggreater{\mathbin{>\!\!\!>}}
\newcommand\llesser{\mathbin{<\!\!\!<}}

\newcommand{\YesV}{\ding{51}}%
\newcommand{\NoX}{\ding{55}}
\DeclareMathSymbol{@}{\mathord}{letters}{"3B}

\newcommand\paren[1]{\left(#1\right)}
\newcommand\abs[1]{\left\lvert#1\right\rvert}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\tuple[1]{\left\langle#1\right\rangle}
\newcommand\inner[2]{\langle #1, #2 \rangle}


\newcommand\crossb[1]{[#1]_\times}


\newcommand\timess{\mathbin{\!\times\!}}

\newcommand\nicebar[1]{\mkern 4mu\overline{\mkern-4mu#1}}

\newcommand\yourname[1]{\textcolor{blue}{Name says: #1}}

\newcommand\mypara[1]{\vspace{1mm}\noindent\textbf{#1}}

\def\rot#1{\rotatebox{90}{#1}}

\def\latex/{\LaTeX}
\def\bibtex/{\hologo{BibTeX}}


% \newcommand\PD[2]{\frac{\partial #1}{\partial #2}}
\newcommand\adj[2]{\overline{ #1}_{#2}}

\newcommand {\dylan}[1]{{\color{red}\textbf{?DT: }#1}\normalfont}
\newcommand {\animesh}[1]{{\color{orange}\textbf{?AG: }#1}\normalfont}
\newcommand {\tony}[1]{{\color{blue}\textbf{?Tony: }#1}\normalfont}


==> tex/intro_for_abstract.tex <==
Hands are the primary tools through which humans interact with the physical world, and it is responsible for most of the intricate and complex manipulation of objects.
% \dylan{Q: Have we decided on Hand-Object Interaction instead of Hand-Object Pose Estimation throughout?}
A good understanding of hand-object interaction helps with many learning-based tasks like action recognition,
robotic manipulation,
user interaction, etc.  

Estimating hand and object interaction presents several challenges.
Firstly, the complex, deformable geometry and dynamics of hands make learning and optimization difficult.    
Unlike rigid objects, human hands are articulated with joints and possess a high degree of freedom.
Their nonlinearity and nonconvexity only add to the complexity of the task.
Secondly, the presence of heavy occlusions both within and between hands and objects creates ambiguity when predicting hand poses during manipulation.
Finally, the rich contact between hands and objects in interaction scenes necessitates the need for a consistent estimation of both hand and object to avoid penetration.

There are generally two categories of approaches for estimating hand and object poses. The first category is the purely learning-based approach, in which researchers carefully design network architectures, loss functions, and training strategies to learn a generalizable mapping from images to hand and object configurations~\cite{hasson19_obman,liu2021semi}.
% \dylan{Todo: choose subset of related works citations, maybe ObMan, photometric consistency, interactions in time}
Although neural networks and large training datasets can mitigate the difficulties posed by high degrees of freedom and non-convexity, they cannot guarantee interpretability or correctness. The second category of approaches is optimization-based~\cite{rhoi2020,hasson20_handobjectconsist},
% \dylan{Todo: subset of related works. perhaps Hasson 3DV21, In the Wild, HO3D itself} 
which involves defining and optimizing heuristic target functions to improve physical feasibility and reduce penetrations. Although the optimization process may be slower, per-frame iterations can improve the accuracy of the results. % However, it is worth noting that many optimization-based approaches are open-loop, which means that the optimized results may differ from the original input.

In this paper, we take advantage of both learning and optimization techniques. Our method leverages pre-trained networks to provide an initial estimate of the poses, and then uses differentiable self-supervised terms to further refine the estimation by correcting errors in pixel-level misalignment and non-physical penetration/oscillation. Inspired by the success of self-supervised learning in large-scale vision and language models~\cite{brown2020language}, we aim to adopt similar techniques to estimate hand-object interactions. Specifically, we propose supervising the pose prediction by comparing it with subsequent video frames, which is similar to how text generation can be trained using sequence completion.

To enable the backpropagation of gradients from the image space, we develop fully-differentiable operators that simulate and render predicted poses. This closed-loop optimization approach helps improve the accuracy of the estimation, making it closer to the input image. We also incorporate several regularization terms to minimize motion oscillation and collision in predicted sequences. 

While the optimization process improves accuracy, it can be time-consuming. To address this issue, we present an alternative filtering technique, such as the Kalman filter~\cite{ribeiro2004kalman}, to further utilize our differentiable dynamics and observation modules. This approach allows users to make a trade-off between efficiency and accuracy, depending on whether they choose to perform online tracking or offline optimization. Within this integrated differentiable rendering and simulation pipeline, we also apply our pose estimation to human and synthetic robot hand scenes, demonstrating the generalizability and robustness of our method. Figure~\ref{fig:teaser} summarizes several applications of this approach.

\vspace*{0.25em}
In summary, the key contributions of this work are:
%\vspace{-\topsep}
\begin{itemize}
\setlength{\itemsep}{1mm}
\setlength{\parskip}{0pt}
    \item An integrated differentiable rendering and simulation pipeline to estimate the hand-object interaction. 
    \item Both offline optimization and online tracking processes that can predict poses and contact information, providing users with options to balance between accuracy and efficiency. 
    \item Experiments that generalize our priors to applications, including contact refinement, robotic hand, and human bodies.
\end{itemize}

In our experiments, our method can achieve comparable or better pose estimation results in hand-object-interaction datasets~\cite{hampali2020honnotate,hampali2022keypointtransformer}. Additionally, we show that the contact information predicted by our method can effectively refine pose estimation. Our ablation study compares the differences between the optimization and tracking results, further validating the contributions of different losses.

==> tex/methods_backup.tex <==


Our approach assumes a known object model and estimates physically plausible hand-object pose from a monocular video with a sequence of RGB images. 
%
Figure x illustrates the overview of our pipeline. In this section, we describe the two main components of our method: differentiable rendering for hand-object pose estimation and physics simulation for realistic hand-object interaction.



%

% \subsection{Hand-object pose estimation} 
\subsection{Differentiable Rendering Priors} 
%
The first component of our approach involves jointly estimating hand and object pose using differentiable rendering.
%
In particular, we represent the hand using the MANO~\cite{MANO:SIGGRAPHASIA:2017} hand model, which maps hand pose $(\theta\in R^{45})$ and shape $(\beta\in R^{45})$ parameters to 3d hand vertices through the following equation: $V_{hand}=MANO(\theta, \beta)$. 
%
We represent the object using the 6DoF representation, which contains the global translation $(T_{obj}\in R^{3})$ and rotation $(R_{obj}\in R^{3})$. 
%
We initialized hand and object poses through a state-of-the-art learning-based model~\cite{liu2021semi} from a sequence of RGB images.
%
\paragraph{\textbf{Segmentation detection}} Instance segmentation is the key information we rely on to further optimize hand and object poses. 
%
We use a segmentation detector~\cite{Kirillov_2020_pointrend} trained on the COCO dataset~\cite{Lin_coco_2014} to extract hand and object masks.
%
Our experiment shows that though Pointrend was not trained on YCB objects, it can always correctly detect object masks if we ignore the classification information.
%
 However, it is not the case for hands, as fingertips are harder to detect.
 %
 Thus, we further trained Pointrend to obtain better masks of hand and hand-hold objects.
 %
\paragraph{\textbf{Optimization}} For each frame, we utilized a differentiable rendering tool~\cite{liu2019softras} that project 3D hand-object vertices to 2D,then optimized hand parameters $(\theta, \beta, T_{hand}, R_{obj})$ and object parameters $(T_{obj}, R_{obj})$ by fitting the projected vertices into hand and object masks.
%
To ensure continuity across frames, we formulate the image error and several continuity errors into a differentiable equation, then minimize the loss using gradient descent. 
%
Next, we describe loss terms we used in optimization:
%
\paragraph{\textbf{Image loss $(L_{img})$}} As hand texture is unavailable, we use differentiable renderer to render only the object in the camera coordinate then applied L2 loss between the rendered image $(I_{r})$ and the input RGB image$(I_{in})$ cropped by the detected object mask $(M_{obj})$. 
%
As this loss term is occlusion aware~\cite{zhang2020phosa}, we did not penalize mismatch happens in the hand occlude region $(M_{hand})$ as in~\cite{hasson20_handobjectconsist}. 
%
The image loss term can be expressed as follow:
%
\begin{equation}
    L_{img} = \lVert (1 - M_{hand})I_r - M_{obj}I_{in} \rVert_{2}^{2}
\end{equation}
%
Through our experiment, we found that this loss term only plays a positive row in limited situations, due to the limitation of lighting conditions and textures.
%
\paragraph{\textbf{Mask loss $(L_{mask})$}} We use differentiable renderer to render the hand and object together in the camera coordinate then applied L2 loss between the rendered mask  $(M_{r})$ and the detected mask $(M_{d})$.
%
The mask loss term can be expressed as follow:
%
\begin{equation}
     L_{mask} = \lVert M_{r} - M_{d} \rVert_{2}^{2}
\end{equation}
%
\paragraph{\textbf{Scale loss $(L_{scale})$}} Similar to~\cite{hasson20_handobjectconsist}, we allow the object to be scaled.
%
We penalize object scales that deviate from their original scale level.
%
\paragraph{Continuity loss $(L_{con})$} To ensure the continuity of hand and object across frames, we penalized the sudden change of object and hand in two consecutive frames. 
%
For object, we applied L2 loss between object vertices in current frame $(V_t)$ and previous frame ($V_(t-1)$). 
%
For hand, we applied L2 loss between hand pose in current frame $(\theta_t)$ and previous frame $(\theta_{t-1})$.
%


\subsection{Differentiable Physics Priors}

The continuity loss term can be expressed as follow:
%
\begin{equation}
     L_{con} = \lambda_1\lVert V_t - V_{t-1} \rVert_{2}^{2} + \lambda_2\lVert \theta_t - \theta_{t-1} \rVert_{2}^{2}
\end{equation}
%
\paragraph{\textbf{Smoothness loss $(L_{smo})$}} During experiment, we empirically discovered that objects usually have sudden shaking across several frames. 
%
Thus, we added a smoothness loss term to punish the sudden changes of object velocity. 
%
Specifically, we applied L2 loss on object displacement across three consecutive frames.
%
The smoothness loss term can be expressed as follow:
%
\begin{equation}
     L_{smo} = \lVert (V_t - V_{t-1}) - (V_{t-1} - V_{t-2}) \rVert_{2}^{2}
\end{equation}
%
\paragraph{\textbf{Sliding loss $(L_{sli})$}} Some sentences


The final loss equation is a weighted combination of all previous described terms, where the weight of each term is set empirically through experiment.
